When Rewards Disagree: Reward Weighting for Token-Efficient Video Reasoning

Human perception interprets video dynamics by constructing structured mental representations of entities, actions, and temporal boundaries before engaging in high-level reasoning. In contrast, current Video-LLMs typically rely on unstructured Chain-of-Thought (CoT), where crucial visual cues are obscured by verbose narration. While recent efforts ground reasoning in intermediate visual evidence, they rely on task-specific schemas that fail to generalize across diverse video understanding tasks. To address this, we introduce Structured Event Evidence, a unified, temporally ordered schema designed for general video reasoning. However, post-training a model to extract structured evidence while reasoning introduces a severe multi-objective optimization bottleneck, as candidate rollouts must simultaneously satisfy schema compliance, task accuracy, and reasoning budget. Standard reinforcement learning (RL) algorithms attempt to balance these objectives via static scalarization, enforcing a rigid accuracy-length trade-off across training and obscuring fine-grained reward signals. We resolve this by proposing Group-Relative Advantage Balancing (GRAB), which dynamically computes Pareto-optimal objective weights within each rollout group via a minimum-norm criterion over centered rewards. Operating strictly in reward space, GRAB incurs virtually zero computational overhead (<0.002% relative runtime to GRPO) and eliminates brittle weight tuning. Supported by our new PARSE-60K dataset (60K annotations across 35K videos) and a three-stage progressive curriculum, we train PARSE-4B. Across temporal grounding and video question-answering benchmarks, GRAB generates 13% to 39% fewer tokens while maintaining competitive accuracy with exhaustively hand-tuned static weights -- without requiring hyperparameter weight sweeps.

==> tables/frozen_format.tex <==
% Falsification run: format reward frozen at 1.0 in Stage 3, so |V| <= 2 holds in
% every group and GRAB should reduce to uniform-weight GRPO.
% The first two rows are the unfrozen runs copied from Table 1 at the same group
% size, kept here so the collapse is visible without turning back.
% Nothing is bolded: the point of the lower block is that the two rows agree.
\begin{table}[H]
\centering
\resizebox{0.72\linewidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Run ($G=8$)} & \textbf{R1@0.3} & \textbf{R1@0.5} & \textbf{R1@0.7} & \textbf{Len} \\ \midrule
GRPO & 57.2 & 38.3 & 19.4 & 842 \\
\method{} & 59.1 & 41.1 & 21.6 & 503 \\ \midrule
GRPO, format frozen & 57.0 & 38.3 & 20.0 & 851 \\
\method{}, format frozen & 57.3 & 38.4 & 19.5 & 838 \\ \bottomrule
\end{tabular}
}
\vspace{1em}
\caption{Freezing the format reward at $1.0$ forces at most two live objectives in
every group, where \method{} and uniform-weight GRPO are the same update. The lower
block is the test and the two rows agree to within half a point. The upper block
repeats the unfrozen runs from Table~\ref{tab:ablation} at the same group size,
where the third objective is available and the gap is present. All runs use
Charades-TimeLens.}
\label{tab:frozen_format}
\end{table}


==> tables/second_backbone.tex <==
% Second backbone. The + GRAB row is the one already in Table 3; the base and
% + GRPO rows are what turn it into a controlled comparison. Len comes from the
% same evaluation pass, so it costs nothing extra.
\begin{table}[H]
\centering
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Model} & \textbf{RAR} & \textbf{ECA} & \textbf{RVQ} & \textbf{TVG} & \textbf{GVQ} & \textbf{VideoMME} & \textbf{Len} \\ \midrule
Qwen2.5-VL-3B                & 38.4 & 47.2 & 52.2 & 19.9 & 55.1 & 61.5 & -- \\
Qwen2.5-VL-3B + GRPO         & --   & --   & --   & --   & --   & --   & -- \\
\textbf{Qwen2.5-VL-3B + \method{}} & \textbf{42.7} & \textbf{50.4} & \textbf{54.1} & \textbf{32.0} & \textbf{55.7} & \textbf{64.0} & -- \\ \bottomrule
\end{tabular}
}
\vspace{1em}
\caption{\method{} on a second backbone. The GRPO row is the control that separates
the algorithm from the PARSE-60K curriculum, since both RL runs start from the
same checkpoint and see the same data.}
\label{tab:second_backbone}
\end{table}

